Leveraging Large Language Models to Develop Heuristics for Emerging Optimization Problems

Combinatorial optimization problems often rely on heuristic algorithms to generate efficient solutions. However, the manual design of heuristics is resource-intensive and constrained by the designer's expertise. Recent advances in artificial intelligence, particularly large language models (LLMs), have demonstrated the potential to automate heuristic generation through evolutionary frameworks. Recent works focus only on well-known combinatorial optimization problems like the traveling salesman problem and online bin packing problem when designing constructive heuristics. This study investigates whether LLMs can effectively generate heuristics for niche, not yet broadly researched optimization problems, using the unit-load pre-marshalling problem as an example case. We propose the Contextual Evolution of Heuristics (CEoH) framework, an extension of the Evolution of Heuristics (EoH) framework, which incorporates problem-specific descriptions to enhance in-context learning during heuristic generation. Through computational experiments, we evaluate CEoH and EoH and compare the results. Results indicate that CEoH enables smaller LLMs to generate high-quality heuristics more consistently and even outperform larger models. Larger models demonstrate robust performance with or without contextualized prompts. The generated heuristics exhibit scalability to diverse instance configurations.

==> sources.tex <==
@incollection{casertaContainerRehandlingMaritime2011,
	series = {Operations {Research}/{Computer} {Science} {Interfaces} {Series}},
	title = {Container {Rehandling} at {Maritime} {Container} {Terminals}},
	abstract = {In this paper, we review recent contributions dealing with the rehandling of containers at maritime container terminals. The problems studied in the paper refer to a post-stacking situation, i.e. problems arising after the stacking area has already been arranged. In order to increase efficiency of loading/unloading operations, once updated information about the state of the containers as well as of the vessels becomes available, it is possible to reshuffle the container yard, or a portion of it, in such a way that future loading operations are carried out with maximal efficiency. The increase in efficiency of loading/unloading operations has a bearing on the berthing time of the vessels, which, in turn, is a widely accepted indicator of port efficiency. Three types of post-stacking problems have been identified, namely (i) the remarshalling problem, (ii) the premarshalling problem, and (iii) the relocation problem. With respect to each of these problems, a thorough explanation of the problem itself, its relevance and its connections with other container handling issues are offered. In addition, algorithmic approaches to tackle such problems are summarized.},
	urldate = {2021-08-09},
	booktitle = {Handbook of {Terminal} {Planning}},
	author = {Caserta, Marco and Schwarze, Silvia and Voß, Stefan},
	year = {2011},
	keywords = {Container Terminal, Export Container, Container Handling, Stowage Plan, Target Container},
	pages = {247-269},
        doi = {10.1007/978-1-4419-8408-1_13  }
}

@Article{Tierney2017,
    author={Tierney, Kevin
    and Pacino, Dario
    and Vo{\ss}, Stefan},
    title={Solving the pre-marshalling problem to optimality with A* and IDA*},
    journal={Flexible Services and Manufacturing Journal},
    year={2017},
    month={Jun},
    day={01},
    volume={29},
    number={2},
    pages={223-259},
    issn={1936-6590},
    doi={10.1007/s10696-016-9246-6},
    url={https://doi.org/10.1007/s10696-016-9246-6}                        
}

@article{stentoft2021drivers,
  title={Drivers and barriers for Industry 4.0 readiness and practice: empirical evidence from small and medium-sized manufacturers},
  author={Stentoft, Jan and Adsb{\o}ll Wickstr{\o}m, Kent and Philipsen, Kristian and Haug, Anders},
  journal={Production Planning \& Control},
  volume={32},
  number={10},
  pages={811--828},
  year={2021},
  publisher={Taylor \& Francis}
}
@article{kamble2018analysis,
  title={Analysis of the driving and dependence power of barriers to adopt industry 4.0 in Indian manufacturing industry},
  author={Kamble, Sachin S and Gunasekaran, Angappa and Sharma, Rohit},
  journal={Computers in Industry},
  volume={101},
  pages={107--119},
  year={2018},
  publisher={Elsevier}
}

@misc{geissbauer2016industry,
  title={Industry 4.0: Building the digital enterprise},
  author={Geissbauer, Reinhard and Vedso, Jesper and Schrauf, Stefan},
  year={2016}
}

@misc{geissbauer2022digital,
  title={PwC Digital Factory Transformation Survey 2022},
  author={Geissbauer, Reinhard and Bruns, Michael and Wunderlin, Jens}, 
  year={2022}
}

@article{glass2018identifying,
  title={Identifying the barriers to Industrie 4.0},
  author={Glass, Rupert and Meissner, Alyssa and Gebauer, Christopher and St{\"u}rmer, Sandra and Metternich, Joachim},
  journal={Procedia Cirp},
  volume={72},
  pages={985--988},
  year={2018},
  publisher={Elsevier}
}

@article{horvath2019driving,
  title={Driving forces and barriers of Industry 4.0: Do multinational and small and medium-sized companies have equal opportunities?},
  author={Horv{\'a}th, D{\'o}ra and Szab{\'o}, Roland Zs},
  journal={Technological forecasting and social change},
  volume={146},
  pages={119--132},
  year={2019},
  publisher={Elsevier}
}

@article{shafto2012modeling,
  title={Modeling, simulation, information technology \& processing roadmap},
  author={Shafto, Mike and Conroy, Mike and Doyle, Rich and Glaessgen, Ed and Kemp, Chris and LeMoigne, Jacqueline and Wang, Lui},
  journal={National Aeronautics and Space Administration},
  volume={32},
  number={2012},
  pages={1--38},
  year={2012}
}

@article{kuehner2021digital,
  title={Digital twin: finding common ground--a meta-review},
  author={Kuehner, Kim Jessica and Scheer, Richard and Strassburger, Steffen},
  journal={Procedia CIRP},
  volume={104},
  pages={1227--1232},
  year={2021},
  publisher={Elsevier}
}

@phdthesis{davis1985technologyTAM1,
  title={A technology acceptance model for empirically testing new end-user information systems: Theory and results},
  author={Davis, Fred D},
  year={1985},
  school={Massachusetts Institute of Technology}
}

@article{venkatesh2000TAM2,
  title={A theoretical extension of the technology acceptance model: Four longitudinal field studies},
  author={Venkatesh, Viswanath and Davis, Fred D},
  journal={Management science},
  volume={46},
  number={2},
  pages={186--204},
  year={2000},
  publisher={INFORMS}
}

@article{venkatesh2008TAM3,
  title={Technology acceptance model 3 and a research agenda on interventions},
  author={Venkatesh, Viswanath and Bala, Hillol},
  journal={Decision sciences},
  volume={39},
  number={2},
  pages={273--315},
  year={2008},
  publisher={Wiley Online Library}
}

@article{venkatesh2003UTAUT,
  title={User acceptance of information technology: Toward a unified view},
  author={Venkatesh, Viswanath and Morris, Michael G and Davis, Gordon B and Davis, Fred D},
  journal={MIS quarterly},
  pages={425--478},
  year={2003},
  publisher={JSTOR}
}

@article{muller2021industrial,
  title={Industrial autonomous systems: a survey on definitions, characteristics and abilities},
  author={M{\"u}ller, Manuel and M{\"u}ller, Timo and Ashtari Talkhestani, Behrang and Marks, Philipp and Jazdi, Nasser and Weyrich, Michael},
  journal={at-Automatisierungstechnik},
  volume={69},
  number={1},
  pages={3--13},
  year={2021},
  publisher={De Gruyter Oldenbourg}
}

@article{wanner2022effect,
  title={The effect of transparency and trust on intelligent system acceptance: Evidence from a user-based study},
  author={Wanner, Jonas and Herm, Lukas-Valentin and Heinrich, Kai and Janiesch, Christian},
  journal={Electronic Markets},
  pages={1--24},
  year={2022},
  publisher={Springer}
}

@article{nastjuk2020drives,
  title={What drives the acceptance of autonomous driving? An investigation of acceptance factors from an end-user's perspective},
  author={Nastjuk, Ilja and Herrenkind, Bernd and Marrone, Mauricio and Brendel, Alfred Benedikt and Kolbe, Lutz M},
  journal={Technological Forecasting and Social Change},
  volume={161},
  pages={120319},
  year={2020},
  publisher={Elsevier}
}

@article{davis2004toward,
  title={Toward preprototype user acceptance testing of new information systems: implications for software project management},
  author={Davis, Fred D and Venkatesh, Viswanath},
  journal={IEEE Transactions on Engineering management},
  volume={51},
  number={1},
  pages={31--46},
  year={2004},
  publisher={IEEE}
}





@article{ghazizadeh2012extending,
  title={Extending the Technology Acceptance Model to assess automation},
  author={Ghazizadeh, Mahtab and Lee, John D and Boyle, Linda Ng},
  journal={Cognition, Technology \& Work},
  volume={14},
  pages={39--49},
  year={2012},
  publisher={Springer}
}

@article{bagozzi2007legacy,
  title={The legacy of the technology acceptance model and a proposal for a paradigm shift.},
  author={Bagozzi, Richard P},
  journal={Journal of the association for information systems},
  volume={8},
  number={4},
  pages={3},
  year={2007}
}

@article{burton2020systematic,
  title={A systematic review of algorithm aversion in augmented decision making},
  author={Burton, Jason W and Stein, Mari-Klara and Jensen, Tina Blegind},
  journal={Journal of Behavioral Decision Making},
  volume={33},
  number={2},
  pages={220--239},
  year={2020},
  publisher={Wiley Online Library}
}

@book{fishbein1975TRA,
author = {Fishbein, M. and Ajzen, Icek},
year = {1975},
month = {05},
pages = {},
title = {Belief, attitude, intention and behaviour: An introduction to theory and research},
volume = {27}
}

@book{rogers2010diffusion,
  title={Diffusion of innovations},
  author={Rogers, Everett M},
  year={2010},
  publisher={Simon and Schuster}
}

@article{KAMAL2020101212,
title = {Investigating acceptance of telemedicine services through an extended technology acceptance model (TAM)},
journal = {Technology in Society},
volume = {60},
pages = {101212},
year = {2020},
issn = {0160-791X},
doi = {https://doi.org/10.1016/j           .techsoc.2019.101212},
url = {https://www.sciencedirect.com/science/article/pii/S0160791X19300909},
author = {Syeda Ayesha Kamal and Muhammad Shafiq and Priyanka Kakria},
keywords = {Telemedicine, Technology acceptance, Usage intention, TAM, Developing countries, PLS},
}

@article{harst2019theories,
  title={Theories predicting end-user acceptance of telemedicine use: systematic review},
  author={Harst, Lorenz and Lantzsch, Hendrikje and Scheibe, Madlen},
  journal={Journal of medical Internet research},
  volume={21},
  number={5},
  pages={e13117},
  year={2019},
  publisher={JMIR Publications Toronto, Canada}
}

@article{ahmad2018review,
  title={Review of the technology acceptance model (TAM) in internet banking and mobile banking},
  author={Ahmad, Maqbool},
  journal={International Journal of Information Communication Technology and Digital Convergence},
  volume={3},
  number={1},
  pages={23--41},
  year={2018}
}

@article{granic2019technology,
  title={Technology acceptance model in educational context: A systematic literature review},
  author={Grani{\'c}, Andrina and Maranguni{\'c}, Nikola},
  journal={British Journal of Educational Technology},
  volume={50},
  number={5},
  pages={2572--2593},
  year={2019},
  publisher={Wiley Online Library}
}

@article{kaur2018trust,
  title={Trust in driverless cars: Investigating key factors influencing the adoption of driverless cars},
  author={Kaur, Kanwaldeep and Rampersad, Giselle},
  journal={Journal of Engineering and Technology Management},
  volume={48},
  pages={87--96},
  year={2018},
  publisher={Elsevier}
}

@article{jetter2018augmented,
  title={Augmented reality tools for industrial applications: What are potential key performance indicators and who benefits?},
  author={Jetter, J{\'e}rȏme and Eimecke, J{\"o}rgen and Rese, Alexandra},
  journal={Computers in Human Behavior},
  volume={87},
  pages={18--33},
  year={2018},
  publisher={Elsevier}
}

@inproceedings{brohl2016tam,
  title={TAM reloaded: a technology acceptance model for human-robot cooperation in production systems},
  author={Br{\"o}hl, Christina and Nelles, Jochen and Brandl, Christopher and Mertens, Alexander and Schlick, Christopher M},
  booktitle={HCI International 2016--Posters' Extended Abstracts: 18th International Conference, HCI International 2016, Toronto, Canada, July 17-22, 2016, Proceedings, Part I 18},
  pages={97--103},
  year={2016},
  organization={Springer}
}

@inproceedings{lotz2019you,
  title={You’re my mate--acceptance factors for human-robot collaboration in industry},
  author={Lotz, V and Himmel, S and Ziefle, M},
  booktitle={International Conference on Competitive Manufacturing},
  pages={10},
  year={2019}
}

@article{onkal2009relative,
  title={The relative influence of advice from human experts and statistical methods on forecast adjustments},
  author={{\"O}nkal, Dilek and Goodwin, Paul and Thomson, Mary and G{\"o}n{\"u}l, Sinan and Pollock, Andrew},
  journal={Journal of Behavioral Decision Making},
  volume={22},
  number={4},
  pages={390--409},
  year={2009},
  publisher={Wiley Online Library}
}

@article{castelo2019task,
  title={Task-dependent algorithm aversion},
  author={Castelo, Noah and Bos, Maarten W and Lehmann, Donald R},
  journal={Journal of Marketing Research},
  volume={56},
  number={5},
  pages={809--825},
  year={2019},
  publisher={SAGE Publications Sage CA: Los Angeles, CA}
}

@article{lee2004trust,
  title={Trust in automation: Designing for appropriate reliance},
  author={Lee, John D and See, Katrina A},
  journal={Human factors},
  volume={46},
  number={1},
  pages={50--80},
  year={2004},
  publisher={SAGE Publications Sage UK: London, England}
}

@article{wischnewski2023measuring,
  title={Measuring and Understanding Trust Calibrations for Automated Systems: A Survey of the State-Of-The-Art and Future Directions},
  author={Wischneski, MAGDALENA and KR{\"A}MER, NICOLE and M{\"U}LLER, EMMANUEL},
  year={2023}
}


@article{lee1992trust,
  title={Trust, control strategies and allocation of function in human-machine systems},
  author={Lee, John and Moray, Neville},
  journal={Ergonomics},
  volume={35},
  number={10},
  pages={1243--1270},
  year={1992},
  publisher={Taylor \& Francis}
}

@article{dietvorst2015algorithm,
  title={Algorithm aversion: people erroneously avoid algorithms after seeing them err.},
  author={Dietvorst, Berkeley J and Simmons, Joseph P and Massey, Cade},
  journal={Journal of Experimental Psychology: General},
  volume={144},
  number={1},
  pages={114},
  year={2015},
  publisher={American Psychological Association}
}

@article{khastgir2018calibrating,
  title={Calibrating trust through knowledge: Introducing the concept of informed safety for automation in vehicles},
  author={Khastgir, Siddartha and Birrell, Stewart and Dhadyalla, Gunwant and Jennings, Paul},
  journal={Transportation research part C: emerging technologies},
  volume={96},
  pages={290--303},
  year={2018},
  publisher={Elsevier}
}

@article{kraus2019two,
  title={Two routes to trust calibration: effects of reliability and brand information on trust in automation},
  author={Kraus, Johannes Maria and Forster, Yannick and Hergeth, Sebastian and Baumann, Martin},
  journal={International Journal of Mobile Human Computer Interaction (IJMHCI)},
  volume={11},
  number={3},
  pages={1--17},
  year={2019},
  publisher={IGI Global}
}

@article{mcguirl2006supporting,
  title={Supporting trust calibration and the effective use of decision aids by presenting dynamic system confidence information},
  author={McGuirl, John M and Sarter, Nadine B},
  journal={Human factors},
  volume={48},
  number={4},
  pages={656--665},
  year={2006},
  publisher={SAGE Publications Sage CA: Los Angeles, CA}
}

@article{okamura2020adaptive,
  title={Adaptive trust calibration for human-AI collaboration},
  author={Okamura, Kazuo and Yamada, Seiji},
  journal={Plos one},
  volume={15},
  number={2},
  pages={e0229132},
  year={2020},
  publisher={Public Library of Science San Francisco, CA USA}
}

@inproceedings{akash2020toward,
  title={Toward adaptive trust calibration for level 2 driving automation},
  author={Akash, Kumar and Jain, Neera and Misu, Teruhisa},
  booktitle={Proceedings of the 2020 international conference on multimodal interaction},
  pages={538--547},
  year={2020}
}

@phdthesis{seppelt2009supporting,
  title={Supporting operator reliance on automation through continuous feedback},
  author={Seppelt, Bobbie Danielle},
  year={2009},
  school={University of Iowa}
}

@inproceedings{zhang2020effect,
  title={Effect of confidence and explanation on accuracy and trust calibration in AI-assisted decision making},
  author={Zhang, Yunfeng and Liao, Q Vera and Bellamy, Rachel KE},
  booktitle={Proceedings of the 2020 conference on fairness, accountability, and transparency},
  pages={295--305},
  year={2020}
}

@article{chen2018description,
  title={The description-experience gap in the effect of warning reliability on user trust and performance in a phishing-detection context},
  author={Chen, Jing and Mishler, Scott and Hu, Bin and Li, Ninghui and Proctor, Robert W},
  journal={International Journal of Human-Computer Studies},
  volume={119},
  pages={35--47},
  year={2018},
  publisher={Elsevier}
}

@inproceedings{wang2016trust,
  title={Trust calibration within a human-robot team: Comparing automatically generated explanations},
  author={Wang, Ning and Pynadath, David V and Hill, Susan G},
  booktitle={2016 11th ACM/IEEE International Conference on Human-Robot Interaction (HRI)},
  pages={109--116},
  year={2016},
  organization={IEEE}
}

@inproceedings{yang2020visual,
  title={How do visual explanations foster end users' appropriate trust in machine learning?},
  author={Yang, Fumeng and Huang, Zhuanyi and Scholtz, Jean and Arendt, Dustin L},
  booktitle={Proceedings of the 25th International Conference on Intelligent User Interfaces},
  pages={189--201},
  year={2020}
}

@article{wang2022effects,
  title={Effects of explanations in AI-assisted decision making: principles and comparisons},
  author={Wang, Xinru and Yin, Ming},
  journal={ACM Transactions on Interactive Intelligent Systems},
  volume={12},
  number={4},
  pages={1--36},
  year={2022},
  publisher={ACM New York, NY}
}

@article{naiseh2023different,
  title={How the different explanation classes impact trust calibration: The case of clinical decision support systems},
  author={Naiseh, Mohammad and Al-Thani, Dena and Jiang, Nan and Ali, Raian},
  journal={International Journal of Human-Computer Studies},
  volume={169},
  pages={102941},
  year={2023},
  publisher={Elsevier}
}

@inproceedings{lai2019human,
  title={On human predictions with explanations and predictions of machine learning models: A case study on deception detection},
  author={Lai, Vivian and Tan, Chenhao},
  booktitle={Proceedings of the conference on fairness, accountability, and transparency},
  pages={29--38},
  year={2019}
}

@inproceedings{cheng2019explaining,
  title={Explaining decision-making algorithms through UI: Strategies to help non-expert stakeholders},
  author={Cheng, Hao-Fei and Wang, Ruotong and Zhang, Zheng and O'Connell, Fiona and Gray, Terrance and Harper, F Maxwell and Zhu, Haiyi},
  booktitle={Proceedings of the 2019 chi conference on human factors in computing systems},
  pages={1--12},
  year={2019}
}

@article{fottner2021autonomous,
  title={Autonomous systems in intralogistics--state of the art and future research challenges},
  author={Fottner, Johannes and Clauer, Dana and Hormes, Fabian and Freitag, Michael and Beinke, Thies and Overmeyer, Ludger and Gottwald, S and Elbert, Ralf and Sarnow, Tessa and Schmidt, Thorsten and others},
  journal={Journal LOGISTICS RESEARCH},
  year={2021}
}

@article{pfrommer2020autonomously,
  title={Autonomously organized block stacking warehouses: A review of decision problems and major challenges},
  author={Pfrommer, Jakob and Meyer, Anne},
  journal={Logistics Journal: Proceedings},
  volume={2020},
  number={12},
  year={2020}
}

@article{derhami2016simulation,
  title={A simulation model to evaluate the layout for block stacking warehouses},
  author={Derhami, Shahab and Smith, Jeffrey S and Gue, Kevin R},
  year={2016}
}

@inproceedings{pfrommer2022slapstack,
  title={SLAPStack: A Simulation Framework and a Large-Scale Benchmark Use Case for Autonomous Block Stacking Warehouses},
  author={Pfrommer, Jakob and Rinciog, Alexandru and Zahid, Sohaib and Morrissey, Michael and Meyer, Anne},
  booktitle={Computational Logistics: 13th International Conference, ICCL 2022, Barcelona, Spain, September 21--23, 2022, Proceedings},
  pages={291--305},
  year={2022},
  organization={Springer}
}

@article{hoff2015trust,
  title={Trust in automation: Integrating empirical evidence on factors that influence trust},
  author={Hoff, Kevin Anthony and Bashir, Masooda},
  journal={Human factors},
  volume={57},
  number={3},
  pages={407--434},
  year={2015},
  publisher={Sage Publications Sage CA: Los Angeles, CA}
}

@article{mcknight2000trust,
  title={What is trust? A conceptual analysis and an interdisciplinary model},
  author={McKnight, D Harrison and Chervany, Norman L},
  year={2000}
}

@article{mayer1995integrative,
  title={An integrative model of organizational trust},
  author={Mayer, Roger C and Davis, James H and Schoorman, F David},
  journal={Academy of management review},
  volume={20},
  number={3},
  pages={709--734},
  year={1995},
  publisher={Academy of Management Briarcliff Manor, NY 10510}
}

@article{rempel1985trust,
  title={Trust in close relationships.},
  author={Rempel, John K and Holmes, John G and Zanna, Mark P},
  journal={Journal of personality and social psychology},
  volume={49},
  number={1},
  pages={95},
  year={1985},
  publisher={American Psychological Association}
}

@inproceedings{walliser2016application,
  title={Application of a system-wide trust strategy when supervising multiple autonomous agents},
  author={Walliser, James C and de Visser, Ewart J and Shaw, Tyler H},
  booktitle={Proceedings of the Human Factors and Ergonomics Society Annual Meeting},
  volume={60},
  number={1},
  pages={133--137},
  year={2016},
  organization={SAGE Publications Sage CA: Los Angeles, CA}
}

@article{suh2002effect,
  title={Effect of trust on customer acceptance of Internet banking},
  author={Suh, Bomil and Han, Ingoo},
  journal={Electronic Commerce research and applications},
  volume={1},
  number={3-4},
  pages={247--263},
  year={2002},
  publisher={Elsevier}
}

@inproceedings{cheng2008customer,
  title={Customer acceptance of internet banking: integrating trust and quality with UTAUT model},
  author={Cheng, Dong and Liu, Gang and Qian, Cheng and Song, Yuan-Fang},
  booktitle={2008 IEEE International Conference on Service Operations and Logistics, and Informatics},
  volume={1},
  pages={383--388},
  year={2008},
  organization={IEEE}
}

@article{mcknight2002developing,
  title={Developing and validating trust measures for e-commerce: An integrative typology},
  author={McKnight, D Harrison and Choudhury, Vivek and Kacmar, Charles},
  journal={Information systems research},
  volume={13},
  number={3},
  pages={334--359},
  year={2002},
  publisher={INFORMS}
}

@article{venkatesh2022adoption,
  title={Adoption and use of AI tools: a research agenda grounded in UTAUT},
  author={Venkatesh, Viswanath},
  journal={Annals of Operations Research},
  pages={1--12},
  year={2022},
  publisher={Springer}
}

@article{liu2023increasing,
  title={Increasing user trust in optimisation through feedback and interaction},
  author={Liu, Jie and Marriott, Kim and Dwyer, Tim and Tack, Guido},
  journal={ACM Transactions on Computer-Human Interaction},
  volume={29},
  number={5},
  pages={1--34},
  year={2023},
  publisher={ACM New York, NY}
}

@inproceedings{biran2017explanation,
  title={Explanation and justification in machine learning: A survey},
  author={Biran, Or and Cotton, Courtenay},
  booktitle={IJCAI-17 workshop on explainable AI (XAI)},
  volume={8},
  number={1},
  pages={8--13},
  year={2017}
}

@article{parreno2020minimizing,
  title={Minimizing crane times in pre-marshalling problems},
  author={Parre{\~n}o-Torres, Consuelo and Alvarez-Valdes, Ramon and Ruiz, Rub{\'e}n and Tierney, Kevin},
  journal={Transportation Research Part E: Logistics and Transportation Review},
  volume={137},
  pages={101917},
  year={2020},
  publisher={Elsevier}
}

@article{jimenez2023constraint,
  title={A constraint programming approach for the premarshalling problem},
  author={Jim{\'e}nez-Piqueras, Celia and Ruiz, Rub{\'e}n and Parre{\~n}o-Torres, Consuelo and Alvarez-Valdes, Ramon},
  journal={European Journal of Operational Research},
  volume={306},
  number={2},
  pages={668--678},
  year={2023},
  publisher={Elsevier},
  doi={10.1016/j.ejor.2022.07.042}
}

@article{pfrommer2023solving,
  title={Solving the unit-load pre-marshalling problem in block stacking storage systems with multiple access directions},
  author={Pfrommer, Jakob and Meyer, Anne and Tierney, Kevin},
  journal={European Journal of Operational Research},
  year={2023},
  publisher={Elsevier},
  doi ={10.1016/j.ejor.2023.08.044}
}

@article{maniezzo2021stochastic,
  title={Stochastic premarshalling of block stacking warehouses},
  author={Maniezzo, Vittorio and Boschetti, Marco A and Gutjahr, Walter J},
  journal={Omega},
  volume={102},
  pages={102336},
  year={2021},
  publisher={Elsevier}
}

@article{lee2007optimization,
  title={An optimization model for the container pre-marshalling problem},
  author={Lee, Yusin and Hsu, Nai-Yun},
  journal={Computers \& operations research},
  volume={34},
  number={11},
  pages={3295--3313},
  year={2007},
  publisher={Elsevier},
  doi ={10.1016/j.cor.2005.12.006} 
}

@article{parreno2019integer,
  title={Integer programming models for the pre-marshalling problem},
  author={Parre{\~n}o-Torres, Consuelo and Alvarez-Valdes, Ramon and Ruiz, Rub{\'e}n},
  journal={European Journal of Operational Research},
  volume={274},
  number={1},
  pages={142--154},
  year={2019},
  publisher={Elsevier},
  doi= {10.1016/j.ejor.2018.09.048 }
}

@article{exposito2017intelligent,
  title={Intelligent heuristic techniques for the optimization of the transshipment and storage operations at maritime container terminals},
  author={Exp{\'o}sito-Izquierdo, Christopher},
  journal={Inteligencia Artificial},
  volume={20},
  number={60},
  pages={20--23},
  year={2017},
  doi ={10.4114/intartif.vol20iss60pp20-23}
}

@article{bortfeldt2012tree,
  title={A tree search procedure for the container pre-marshalling problem},
  author={Bortfeldt, Andreas and Forster, Florian},
  journal={European Journal of Operational Research},
  volume={217},
  number={3},
  pages={531--540},
  year={2012},
  publisher={Elsevier},
  doi={10.1016/j.ejor.2011.10.005} 
}

@article{prandtstetter2013dynamic,
  title={A dynamic programming based branch-and-bound algorithm for the container pre-marshalling problem},
  author={Prandtstetter, Matthias},
  journal={Technical repot, IT Austrian institute of technology},
  year={2013},
  doi={}
}

@inproceedings{rendl2013constraint,
  title={Constraint models for the container pre-marshaling problem},
  author={Rendl, Andrea and Prandtstetter, Matthias},
  booktitle={ModRef 2013: The Twelfth International Workshop on Constraint Modelling and Reformulation},
  year={2013},
  url={https://api.semanticscholar.org/CorpusID:43049743}
}
}

@article{exposito2012pre,
  title={Pre-marshalling problem: Heuristic solution method and instances generator},
  author={Exp{\'o}sito-Izquierdo, Christopher and Meli{\'a}n-Batista, Bel{\'e}n and Moreno-Vega, Marcos},
  journal={Expert Systems with Applications},
  volume={39},
  number={9},
  pages={8337--8349},
  year={2012},
  publisher={Elsevier}
}

@inproceedings{kang2006planning,
  title={Planning for intra-block remarshalling in a container terminal},
  author={Kang, Jaeho and Oh, Myung-Seob and Ahn, Eun Yeong and Ryu, Kwang Ryel and Kim, Kap Hwan},
  booktitle={Advances in Applied Artificial Intelligence: 19th International Conference on Industrial, Engineering and Other Applications of Applied Intelligent Systems, IEA/AIE 2006, Annecy, France, June 27-30, 2006. Proceedings 19},
  pages={1211--1220},
  year={2006},
  organization={Springer},
  doi={ 10.1007/11779568_128                  }
}

@article{choe2011generating,
  title={Generating a rehandling-free intra-block remarshaling plan for an automated container yard},
  author={Choe, Ri and Park, Taejin and Oh, Myung-Seob and Kang, Jaeho and Ryu, Kwang Ryel},
  journal={Journal of Intelligent Manufacturing},
  volume={22},
  pages={201--217},
  year={2011},
  publisher={Springer},
  doi ={10.1007/s10845-009-0273-y}
}


@inproceedings{park2009planning,
  title={Planning for remarshaling in an automated container terminal using cooperative coevolutionary algorithms},
  author={Park, Kiyeok and Park, Taejin and Ryu, Kwang Ryel},
  booktitle={Proceedings of the 2009 ACM symposium on Applied Computing},
  pages={1098--1105},
  year={2009},
  doi={10.1145/1529282.1529523 }
}

@phdthesis{pfrommer2023sortingdiss,
    author = {Pfrommer, Jakob},
    title = {Sorting Algorithms for Autonomously Organized Block 
    Stacking Warehouse“},
    school = {Technical University of Dortmund},
    year = {2023}
}



@techreport{pfrommerboemer2024data,
  author={Pfrommer, Jakob and Bömer, Thomas},
  title = {Multibay unit-load pre-marshalling problem instances},
  year = {2024}, 
  url = {https://doi.org/10.5281/zenodo.11093870}                    
}

@article{pfrommerboemer2024sorting,
  title={Sorting multibay block stacking storage systems},
  author={Pfrommer, Jakob and B{\"o}mer, Thomas and Akizhanov, Daniyar and Meyer, Anne},
  journal={arXiv preprint arXiv:2405.04847}       ,
  year={2024}, 
  doi={10.48550/arXiv.2405.04847}
}

@inproceedings{liu2024evolutionEoH,
  title={Evolution of Heuristics: Towards Efficient Automatic Algorithm Design Using Large Language Model},
  author={Liu, Fei and Xialiang, Tong and Yuan, Mingxuan and Lin, Xi and Luo, Fu and Wang, Zhenkun and Lu, Zhichao and Zhang, Qingfu},
  booktitle={Forty-first International Conference on Machine Learning},
  year={2024}
}

@article{ye2024reevo,
  title={Reevo: Large language models as hyper-heuristics with reflective evolution},
  author={Ye, Haoran and Wang, Jiarui and Cao, Zhiguang and Song, Guojie},
  journal={arXiv preprint arXiv:2402.01145}  ,
  year={2024}
}

@inproceedings{
anonymous2024efficientHERCULES,
title={Efficient Heuristics Generation for Solving Combinatorial Optimization Problems Using Large Language Models},
author={Anonymous},
booktitle={Submitted to The Thirteenth International Conference on Learning Representations},
year={2024},
url={https://openreview.net/forum?id=0fwJMANq9P},
note={under review}
}

@article{romera2024mathematical,
  title={Mathematical discoveries from program search with large language models},
  author={Romera-Paredes, Bernardino and Barekatain, Mohammadamin and Novikov, Alexander and Balog, Matej and Kumar, M Pawan and Dupont, Emilien and Ruiz, Francisco JR and Ellenberg, Jordan S and Wang, Pengming and Fawzi, Omar and others},
  journal={Nature},
  volume={625},
  number={7995},
  pages={468--475},
  year={2024},
  publisher={Nature Publishing Group UK London}
}

@misc{liu2024systematicsurveylargelanguage,
      title={A Systematic Survey on Large Language Models for Algorithm Design}, 
      author={Fei Liu and Yiming Yao and Ping Guo and Zhiyuan Yang and Zhe Zhao and Xi Lin and Xialiang Tong and Mingxuan Yuan and Zhichao Lu and Zhenkun Wang and Qingfu Zhang},
      year={2024},
      eprint={2410.14716},
      archivePrefix={arXiv},
      primaryClass={cs.LG},
      url={https://arxiv.org/abs/2410.14716}, 
}

@article{wu2024evolutionary,
  title={Evolutionary computation in the era of large language model: Survey and roadmap},
  author={Wu, Xingyu and Wu, Sheng-hao and Wu, Jibin and Feng, Liang and Tan, Kay Chen},
  journal={arXiv preprint arXiv:2401.10034},
  year={2024}
}
@article{liu2023algorithmAEL,
  title={Algorithm evolution using large language model},
  author={Liu, Fei and Tong, Xialiang and Yuan, Mingxuan and Zhang, Qingfu},
  journal={arXiv preprint arXiv:2311.15249},
  year={2023}
}

@inproceedings{liu2024largeLMEA,
  title={Large language models as evolutionary optimizers},
  author={Liu, Shengcai and Chen, Caishun and Qu, Xinghua and Tang, Ke and Ong, Yew-Soon},
  booktitle={2024 IEEE Congress on Evolutionary Computation (CEC)},
  pages={1--8},
  year={2024},
  organization={IEEE}
}
@misc{yang2024largelanguagemodelsoptimizersOPRO,
      title={Large Language Models as Optimizers}, 
      author={Chengrun Yang and Xuezhi Wang and Yifeng Lu and Hanxiao Liu and Quoc V. Le and Denny Zhou and Xinyun Chen},
      year={2024},
      eprint={2309.03409},
      archivePrefix={arXiv},
      primaryClass={cs.LG},
      url={https://arxiv.org/abs/2309.03409}, 
}
@misc{huang2024multimodalintegrationboostperformanceMLLM,
      title={How Multimodal Integration Boost the Performance of LLM for Optimization: Case Study on Capacitated Vehicle Routing Problems}, 
      author={Yuxiao Huang and Wenjie Zhang and Liang Feng and Xingyu Wu and Kay Chen Tan},
      year={2024},
      eprint={2403.01757},
      archivePrefix={arXiv},
      primaryClass={cs.AI},
      url={https://arxiv.org/abs/2403.01757}, 
}


@misc{sartori2024metaheuristicslargelanguagemodelsMH-LLM*,
      title={Metaheuristics and Large Language Models Join Forces: Towards an Integrated Optimization Approach}, 
      author={Camilo Chacón Sartori and Christian Blum and Filippo Bistaffa and Guillem Rodríguez Corominas},
      year={2024},
      eprint={2405.18272},
      archivePrefix={arXiv},
      primaryClass={cs.AI},
      url={https://arxiv.org/abs/2405.18272}, 
}

@inproceedings{duflo2019gp,
  title={A gp hyper-heuristic approach for generating tsp heuristics},
  author={Duflo, Gabriel and Kieffer, Emmanuel and Brust, Matthias R and Danoy, Gr{\'e}goire and Bouvry, Pascal},
  booktitle={2019 IEEE International Parallel and Distributed Processing Symposium Workshops (IPDPSW)},
  pages={521--529},
  year={2019},
  organization={IEEE}
}

@article{kwon2020pomo,
  title={Pomo: Policy optimization with multiple optima for reinforcement learning},
  author={Kwon, Yeong-Dae and Choo, Jinho and Kim, Byoungjip and Yoon, Iljoo and Gwon, Youngjune and Min, Seungjai},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={21188--21198},
  year={2020}
}

@article{luo2023neural,
  title={Neural combinatorial optimization with heavy decoder: Toward large scale generalization},
  author={Luo, Fu and Lin, Xi and Liu, Fei and Zhang, Qingfu and Wang, Zhenkun},
  journal={Advances in Neural Information Processing Systems},
  volume={36},
  pages={8845--8864},
  year={2023}
}

@article{yu2024autornet,
  title={AutoRNet: Automatically Optimizing Heuristics for Robust Network Design via Large Language Models},
  author={Yu, He and Liu, Jing},
  journal={arXiv preprint arXiv:2410.17656}      ,
  year={2024}
}

@misc{gemma2_27b,
  author       = {Google},
  title        = {Gemma 2},
  howpublished = {\url{https://ollama.com/library/gemma2:27b}},
}

@misc{qwen2.5-coder_32b,
  author       = {DeepSeek},
  title        = {Qwen2.5-Coder},
  howpublished = {\url{https://ollama.com/library/qwen2.5-coder}},
}

@misc{deepseekV3,
  author       = {DeepSeek},
  title        = {DeepSeek V3},
  howpublished = {\url{https://ollama.com/library/deepseek-v3}},
}

@misc{gpt4o,
  author       = {OpenAI},
  title        = {GPT-4O},
  howpublished = {\url{https://openai.com/research/gpt-4o}},
}


@article{ghomri2009continuous,
  title={Continuous models for single and dual cycle times of a multi aisle automated storage and retrieval system},
  author={GHOMRI, Latefa and Zaki, Sari and GUEZZEN, Amine and Tewfik, SARI},
  journal={IFAC Proceedings Volumes},
  volume={42},
  number={4},
  pages={1061--1066},
  year={2009},
  publisher={Elsevier}
}

@article{yao2023beyond,
  title={Beyond Chain-of-Thought, Effective Graph-of-Thought Reasoning in Language Models},
  author={Yao, Yao and Li, Zuchao and Zhao, Hai},
  journal={arXiv preprint arXiv:2305.16582}  ,
  year={2023}
}

@article{min2023beyond,
  title={Beyond accuracy: Evaluating self-consistency of code large language models with identitychain},
  author={Min, Marcus J and Ding, Yangruibo and Buratti, Luca and Pujar, Saurabh and Kaiser, Gail and Jana, Suman and Ray, Baishakhi},
  journal={arXiv preprint arXiv:2310.14053}    ,
  year={2023}
}

@article{gagliardi2014simulation,
  title={A simulation modeling framework for multiple-aisle automated storage and retrieval systems},
  author={Gagliardi, Jean-Philippe and Renaud, Jacques and Ruiz, Angel},
  journal={Journal of Intelligent Manufacturing},
  volume={25},
  pages={193--207},
  year={2014},
  publisher={Springer}
}

@inproceedings{disselnmeyer2024static,
  title={The Static Buffer Reshuffling and Retrieval Problem for Autonomous Mobile Robots},
  author={Disselnmeyer, Max and B{\"o}mer, Thomas and Pfrommer, Jakob and Meyer, Anne},
  booktitle={International Conference on Computational Logistics},
  pages={18--33},
  year={2024},
  organization={Springer},
  url = {https://doi.org/10.1007/978-3-031-71993-6_2}        
}

@inproceedings{bomer2024sorting,
  title={Sorting Multibay Block Stacking Storage Systems with Multiple Robots},
  author={B{\"o}mer, Thomas and Koltermann, Nico and Pfrommer, Jakob and Meyer, Anne},
  booktitle={International Conference on Computational Logistics},
  pages={34--48},
  year={2024},
  organization={Springer},
    url = {https://doi.org/10.1007/978-3-031-71993-6_3}         
}

@techreport{pfrommerboemer2024data,
  author={Pfrommer, Jakob and Bömer, Thomas},
  title = {Multibay unit-load pre-marshalling problem instances},
  year = {2024}, 
  institution = {TU Dortmund},
  url = {https://doi.org/10.5281/zenodo.11093870}                          
}
@article{wang2024policy,
  title={A policy-based Monte Carlo tree search method for container pre-marshalling},
  author={Wang, Ziliang and Zhou, Chenhao and Che, Ada and Gao, Jingkun},
  journal={International Journal of Production Research},
  volume={62},
  number={13},
  pages={4776--4792},
  year={2024},
  publisher={Taylor \& Francis}
}

@article{hottung2020deep,
  title={Deep learning assisted heuristic tree search for the container pre-marshalling problem},
  author={Hottung, Andr{\'e} and Tanaka, Shunji and Tierney, Kevin},
  journal={Computers \& Operations Research},
  volume={113},
  pages={104781},
  year={2020},
  publisher={Elsevier}
}

@article{burke2013hyper,
  title={Hyper-heuristics: A survey of the state of the art},
  author={Burke, Edmund K and Gendreau, Michel and Hyde, Matthew and Kendall, Graham and Ochoa, Gabriela and {\"O}zcan, Ender and Qu, Rong},
  journal={Journal of the Operational Research Society},
  volume={64},
  number={12},
  pages={1695--1724},
  year={2013},
  publisher={Taylor \& Francis}
}

@article{liu2024systematic,
  title={A systematic survey on large language models for algorithm design},
  author={Liu, Fei and Yao, Yiming and Guo, Ping and Yang, Zhiyuan and Lin, Xi and Tong, Xialiang and Yuan, Mingxuan and Lu, Zhichao and Wang, Zhenkun and Zhang, Qingfu},
  journal={arXiv preprint arXiv:2410.14716}     ,
  year={2024}
}

@book{langdon2013foundations,
  title={Foundations of genetic programming},
  author={Langdon, William B and Poli, Riccardo},
  year={2013},
  publisher={Springer Science \& Business Media}
}

@article{austin2021program,
  title={Program synthesis with large language models},
  author={Austin, Jacob and Odena, Augustus and Nye, Maxwell and Bosma, Maarten and Michalewski, Henryk and Dohan, David and Jiang, Ellen and Cai, Carrie and Terry, Michael and Le, Quoc and others},
  journal={arXiv preprint arXiv:2108.07732}     ,
  year={2021}
}

@article{naveed2023comprehensive,
  title={A comprehensive overview of large language models},
  author={Naveed, Humza and Khan, Asad Ullah and Qiu, Shi and Saqib, Muhammad and Anwar, Saeed and Usman, Muhammad and Akhtar, Naveed and Barnes, Nick and Mian, Ajmal},
  journal={arXiv preprint arXiv:2307.06435}    ,
  year={2023}
}

@article{dat2024hsevo,
  title={HSEvo: Elevating Automatic Heuristic Design with Diversity-Driven Harmony Search and Genetic Algorithm Using LLMs},
  author={Dat, Pham Vu Tuan and Doan, Long and Binh, Huynh Thi Thanh},
  journal={arXiv preprint arXiv:2412.14995}    ,
  year={2024}
}


@article{zheng2025MCTS-AHD,
  title={Monte Carlo Tree Search for Comprehensive Exploration in LLM-Based Automatic Heuristic Design},
  author={Zheng, Zhi and Xie, Zhuoliang and Wang, Zhenkun and Hooi, Bryan},
  journal={arXiv preprint arXiv:2501.08603}   ,
  year={2025}
}
